Enabling Cross-Camera Collaboration for Video Analytics on Distributed Smart Cameras

Overlapping cameras offer exciting opportunities to view a scene from different angles, allowing for more advanced, comprehensive and robust analysis. However, existing visual analytics systems for multi-camera streams are mostly limited to (i) per-camera processing and aggregation and (ii) workload-agnostic centralized processing architectures. In this paper, we present Argus, a distributed video analytics system with cross-camera collaboration on smart cameras. We identify multi-camera, multi-target tracking as the primary task of multi-camera video analytics and develop a novel technique that avoids redundant, processing-heavy identification tasks by leveraging object-wise spatio-temporal association in the overlapping fields of view across multiple cameras. We further develop a set of techniques to perform these operations across distributed cameras without cloud support at low latency by (i) dynamically ordering the camera and object inspection sequence and (ii) flexibly distributing the workload across smart cameras, taking into account network transmission and heterogeneous computational capacities. Evaluation of three real-world overlapping camera datasets with two Nvidia Jetson devices shows that Argus reduces the number of object identifications and end-to-end latency by up to 7.13x and 2.19x (4.86x and 1.60x compared to the state-of-the-art), while achieving comparable tracking quality.

==> sections/02_related_work_.tex <==
\section{Related Work}~\label{sec:related_work}
%\subsection{Cross-Camera Collaboration Systems}

%Several systems have been proposed to take benefit from multi-camera collaboration. They focus on different purposes; enriched video analytics, resource efficiency, and distributed processing. 

\parjump \noindent \textbf{Enriched video analytics.} One direction for cross-camera collaboration is to provide enriched, combined video analytics from different viewpoints of multiple cameras~\cite{liu2019caesar,li2020cmcaot,jha2021visage}. Liu et al. developed Caesar~\cite{liu2019caesar}, a system that detects cross-camera complex activities, e.g., a person walking in one camera and talking to another person later in a different camera, by designing abstraction for those activities and combining DNN-based activity detection from non-overlapping cameras. Li et al. presented a camera collaboration system~\cite{li2020cmcaot} that performs active object tracking by exploiting the intrinsic relationship among the poses of cameras. Jha et al. developed Visage~\cite{jha2021visage} that provides 3D image analytics from multiple video streams on drones. \cm{we can add our aichallengeiot paper.} Our work can serve as an underlying on-camera framework of these works, providing multi-camera, multi-task tracking as a primitive task on distributed smart cameras.

\iffalse
\begin{table*}[pt]
\caption{Comparison of cross-camera collaboration approach in \system{} with CrossRoI~\cite{guo2021crossroi} and Spatula~\cite{jain2020spatula}.}
\vspace{-3pt}
\label{tab:comparison}
\begin{tabular}{|p{0.23\linewidth}|p{0.23\linewidth}|p{0.23\linewidth}|p{0.23\linewidth}|}
\hline
& \textbf{Spatula}~\cite{jain2020spatula} & \textbf{CrossRoI}~\cite{guo2021crossroi} & \textbf{Argus (Ours)} \\ \hline
\textbf{Target environment} & Non-overlapping cameras & Overlapping cameras & Overlapping cameras \\ \hline
\textbf{Optimization goal} & Communication and on-server computation costs  & Communication and on-server computation costs & End-to-end latency on cameras  \\ \hline
\textbf{Collaboration granularity} & Cameras  & Areas (RoIs)  & Objects \\ \hline
\textbf{Approach} & Identify the subset of cameras that capture target objects & Find the smallest RoI that contains the target objects & Minimise the number of identification operations across cameras \\ \hline
\textbf{Video processing} & Centralized & Centralized & Distributed \\ \hline
\end{tabular}
\end{table*}
\fi

\parjump \noindent \textbf{Resource efficiency.} Another direction for cross-camera collaboration is to reduce the computational and communication costs of multiple video streams by exploiting their spatial and temporal correlation~\cite{jain2019scaling,jain2020spatula,guo2021crossroi}. Spatula~\cite{jain2019scaling,jain2020spatula} is a cross-camera collaboration system for wide-area camera networks with \emph{non-overlapping} cameras and limits the amount of video data and corresponding communication to be analysed by identifying only those cameras and frames that are likely to contain the target objects. REV~\cite{xu2022rev} also aims at reducing the number of cameras processed by incrementally searching the cameras within the overlapping group and opportunistically skipping processing the rest as soon as the target has been detected. CrossRoI~\cite{guo2021crossroi} and \revise{ Polly~\cite{li2023polly}} leverages spatial correlation to extract the minimum-sized RoI from overlapping cameras and reduces processing and transmission costs by filtering out unmasked RoIs. All such works share the same high-level goal as \system{} in that they leverage spatio-temporal correlation from multiple cameras, but \system{} differs in several aspects, as shown in Table~\ref{tab:comparison}.
%\cm{revisit after working section 3}. \cm{we also need to mention that Spatula and CrossRoI do not have distributed processing capability.}

\parjump \noindent \textbf{Distributed processing.} There have been several attempts to distribute video analytics workloads from large-scale video data into multiple cameras~\cite{hung2018videoedge,zeng2020distream}. VideoEdge~\cite{hung2018videoedge} optimises the resource-accuracy tradeoff by partitioning the analytics pipeline into hierarchical clusters (cameras, private clusters, public clouds). Distream~\cite{zeng2020distream} adaptively balances the workloads across smart cameras. Although these works provided a foundation for designing distributed video analytics systems, they mostly focused on the single-camera video analytics pipeline as the main workload. In this work, we identify that multi-camera, multi-target tracking is a primary, underlying task for overlapping cameras, and propose on-camera distributed processing strategy tailed to it.

%\subsection{On-Device Video Analytics} 
%
%Many video analytics systems have been proposed to efficiently process a large volume of video data on low-end cameras.
%% by adopting on-camera frame filtering~\cite{hsieh2018focus,li2020reducto,xu2021diva}, pipeline adaptation~\cite{apicharttrisorn2019marlin,yi2020eagleeye}, and dynamic adjustment of video resolution~\cite{du2020dds,liu2019edge}. 
%On-camera frame filtering techniques filter out compute-intensive AI model execution in the early stage, e.g., dynamically adapting filtering decisions~\cite{li2020reducto}, leveraging cheap CNN classifiers~\cite{hsieh2018focus}. 
%Yi et al. presented EagleEye~\cite{yi2020eagleeye}, a pipeline adaptation system for person identification which selectively uses different face detection models depending on the quality of face images. 
%%Apicharttrisorn et al. proposed 
%% MARLIN~\cite{apicharttrisorn2019marlin} has been proposed to selectively perform a deep neural network for energy-efficient object tracking. 
%Several attempts have been made to dynamically adjust video resolution to optimise the network bandwidth consumption to enable low-latency offloading~\cite{liu2019edge}, and to optimise video streaming protocol~\cite{du2020dds}. 
%%  The other approach for efficient processing is to optimally schedule DNN inferences from multiple video streams on the GPU cluster~\cite{zhang2017videostorm,jiang2018chameleon,shen2019nexus}.
% 
%While these works manage to achieve a remarkable performance improvement, their attempts are mostly focused on a single camera (or its server). Unlike these works, we target the environment where multiple cameras are installed nearby and focus on optimising the cross-camera operations by leveraging the spatio/temporal association of objects. \system{} can further improve system-wide resource efficiency by adopting these techniques. 



